Attacker Profiling Through Analysis of Attack Patterns in Geographically Distributed Honeypots

Honeypots are a well-known and widely used technology in the cybersecurity community, where it is assumed that placing honeypots in different geographical locations provides better visibility and increases effectiveness. However, how geolocation affects the usefulness of honeypots is not well-studied, especially for threat intelligence as early warning systems. This paper examines attack patterns in a large public dataset of geographically distributed honeypots by answering methodological questions and creating behavioural profiles of attackers. Results show that the location of honeypots helps identify attack patterns and build profiles for the attackers. We conclude that not all the intelligence collected from geographically distributed honeypots is equally valuable and that a good early warning system against resourceful attackers may be built with only two distributed honeypots and a production server.

==> tables/tab_average_attacks.tex <==
\begin{table}[]
\scriptsize
\renewcommand{\arraystretch}{1.5}
\caption{Average number of attacks per attacker by number of attacked honeypots and services}
\begin{center}
\begin{tabular}{c|rrrrrr}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\makecell[c]{H}}} & \multicolumn{6}{c}{\textbf{Services attacked}} \\
\multicolumn{1}{l}{} & \multicolumn{1}{c}{"S=1"} & \multicolumn{1}{c}{"S=2"} & \multicolumn{1}{c}{"S=3"} & \multicolumn{1}{c}{"S=4"} & \multicolumn{1}{c}{"S=5"} & \multicolumn{1}{c}{S\textgreater{}5} \\
\midrule
=1 & 7.47 & 4.73 & 5.68 & 4.85 & 5.64 & 2,045.53 \\
=2 & 3.90 & 5.43 & 7.72 & 7.40 & 8.87 & 273.32 \\
=3 & 5.81 & 7.68 & 9.04 & 10.17 & 11.83 & 445.53 \\
=4 & 8.59 & 7.31 & 9.19 & 9.12 & 10.99 & 34.58 \\
=5 & 12.51 & 9.73 & 17.93 & 29.54 & 10.92 & 26.70 \\
=6 & 20.19 & 12.84 & 23.83 & 21.23 & 12.51 & 323.05 \\
=7 & 38.20 & 25.76 & 47.19 & 20.20 & 17.55 & 98.44 \\
=8 & 20.64 & 49.23 & 47.04 & 104.94 & 93.24 & 173.82 \\
\bottomrule
\end{tabular}
\label{tab:averageattacks}
\end{center}
\end{table}

==> tables/tab_continent_distribution.tex <==
\begin{table}[tb]
\scriptsize
\renewcommand{\arraystretch}{1.5}
\caption{Distribution of attackers and attacks per continent of origin}
{The distribution of attackers is the total number of attackers originating from a continent over the total number of attackers in the dataset. The distribution of attacks is the total number of attacks originating from a continent over the total number of attacks in the dataset}
\begin{center}
\begin{tabular}{l r r}
\toprule
\makecell[c]{\textbf{Continent}\\\textbf{of Origin}} & \makecell[c]{\textbf{Distribution of}\\\textbf{ Attackers}} & \makecell[c]{\textbf{Distribution of}\\\textbf{Attacks}} \\
\midrule
Asia            &  54.71\%  & 38.19\% \\
Europe          &  16.84\%  &  33\% \\
North America   &  15.13\%  &  17.29\% \\
South America   &   8.12\%  &  1.35\% \\
Africa          &   4.58\%  &  0.79\% \\
Oceania         &   0.47\%  &  0.19\% \\
Antarctica      &   0\%  &  0\% \\
\bottomrule
\end{tabular}
\label{tab:axisacontinents}
\end{center}
\end{table}
